Surgery Obstructions for Seifert Fibered Homology Spheres

We examine surgery on a knot in $S^3$ to determine surgery obstructions to Seifert fibered integral homology spheres. We find such surgery obstructions using Heegaard Floer, Knot Floer homology and the mapping cone formula for computing Heegaard Floer homology of surgery on a knot. Here however, we take a different approach and use the number of singular fibers of a Seifert fibered integral homology sphere, which is the toroidal structure, to find obstructions. This approach allows us to show that genus one knots cannot yield Seifert fibered integral homology spheres with six or more singular fibers. Some other obstructions are also presented for higher genus knots.

==> Akprooftikz.tex <==
\begin{center}
\begin{tikzpicture}
\node[hackennode] (w3) at (0,2) {};
\node[left] at (0,2.25) {$v$};
\node[hackennode] (w3.0) at (-0,2.25) {};
\node[hackennode] (w3.1) at (-0,2.5) {};
\node[hackennode] (w3.2) at (-0,2.75) {};
\node[hackennode] (a) at (-1,1) {};
\node[left] at (-1,1.25) {$a$};
\node[hackennode] (b) at (-2,0) {};
\node[left] at (-2,.25) {$b$};
\node[hackennode] (c) at (1,1) {};
\node[right] at (1,1.25) {$c$};
\node[hackennode] (d) at (2,0) {};
\node[right] at (2,.25) {$d$};

\node[hackennode] (v1) at (-3.75,1) {};
\node[below] at (-3.5,1) {$v_1$};
\node[hackennode] (v2) at (-3,1) {};
\node[below] at (-3,1) {$v_2$};
\node[hackennode] (v3) at (-2,1) {};
\node[below] at (-2,1) {$v_3$};

\node[hackennode] (v4) at (-.5,1) {};
\node[below] at (-.5,1) {$v_4$};
\node[hackennode] (d1) at (-.25,1) {};
\node[hackennode] (d2) at (0,1) {};
\node[hackennode] (d3) at (.25,1) {};
\node[hackennode] (v5) at (.5,1) {};
\node[below] at (.5,1) {$v_{m-3}$};


\node[hackennode] (v8) at (2,1) {};
\node[below] at (2,1) {$v_{m-2}$};
\node[hackennode] (v9) at (3,1) {};
\node[below] at (3,1) {$v_{m-1}$};
\node[hackennode] (v10) at (3.75,1) {};
\node[below] at (3.75,1) {$v_m$};


\draw[thick, blue] (w3) -- (a) -- (b);
\draw[thick, blue] (w3) -- (c) -- (d);
\draw[thick, red] (v1) -- (w3);
\draw[thick, red] (v2) -- (w3);
\draw[thick, red] (v3) -- (w3);
\draw[thick, red] (v4) -- (w3);
\draw[thick, red] (v5) -- (w3);
\draw[thick, red] (v8) -- (w3);
\draw[thick, red] (v9) -- (w3);
\draw[thick, red] (v10) -- (w3);

\node[left] at (-4,2) {$n$};
\node[left] at (-4,1) {$n-k$};
\node[left] at (-4,0) {$n-k-1$};
\node[left] at (-4,-1) {$n-k-2$};

\draw[gray, dashed] (-4,2)--(4,2);
\draw[gray, dashed] (-4,1)--(4,1);
\draw[gray, dashed] (-4,0)--(4,0);
\draw[gray, dashed] (-4,-1)--(4,-1);


\end{tikzpicture}
\end{center}

==> Aktikz.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.6}]
\node[hackennode] (w3) at (0,2) {};
\node[left] at (0,2.25) {$v$};
\node[hackennode] (a) at (-.5,1) {};
\node[left] at (-.5,1.25) {$a$};
\node[hackennode] (b) at (-1,0) {};
\node[hackennode] (c) at (.5,1) {};
\node[right] at (.5,1.25) {$b$};
\node[hackennode] (d) at (1,0) {};
\node[hackennode] (e) at (1.5,-1) {};
\node[hackennode] (f) at (-1.5,-1) {};
\node[hackennode] (g) at (-2,-2) {};
\node[left] at (-2,-2.25) {$c$};
\node[hackennode] (h) at (2,-2) {};
\node[right] at (2,-2.25) {$d$};


\node[hackennode] (x) at (1.2,-.3) {};
\node[hackennode] (x) at (1.3,-.5) {};
\node[hackennode] (x) at (1.4,-.7) {};
\node[hackennode] (x) at (-1.2,-.3) {};
\node[hackennode] (x) at (-1.3,-.5) {};
\node[hackennode] (x) at (-1.4,-.7) {};


\draw[thick, blue] (w3) -- (a) -- (b);
\draw[thick, blue] (w3) -- (c) -- (d);
\draw[thick, blue] (e) -- (h);
\draw[thick, blue] (f) -- (g);

\node[left] at (-3.5,2) {$n$};
\node[left] at (-3.5,1) {$n-1$};
\node[left] at (-3.5,0) {$n-2$};
\node[left] at (-3.5,-1) {$n-k+1$};
\node[left] at (-3.5,-2) {$n-k$};
\node[left] at (-3.5,-3) {$n-k-1$};

\draw[gray, dashed] (-3.5,2)--(3.5,2);
\draw[gray, dashed] (-3.5,1)--(3.5,1);
\draw[gray, dashed] (-3.5,0)--(3.5,0);
\draw[gray, dashed] (-3.5,-1)--(3.5,-1);
\draw[gray, dashed] (-3.5,-2)--(3.5,-2);
\draw[gray, dashed] (-3.5,-3)--(3.5,-3);

\end{tikzpicture}
\caption{$A_{k}$-structure in graded root}
\label{Akfig}
\end{figure}

==> Branchtikz.tex <==
\begin{figure}[h]
\centering
\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.6}]
\node[hackennode] (w3) at (1,2) {};
\node[left] at (1,2.25) {$a$};
\node[hackennode] (a) at (.5,1) {};
\node[left] at (.5,1.25) {$b$};
\node[hackennode] (b) at (0,0) {};
\node[hackennode] (b1) at (-.5,-1.5) {};
\node[hackennode] (b2) at (-1,-2.5) {};
\node[hackennode] (e1) at (-.1,-.5) {};
\node[hackennode] (e2) at (-.2,-.8) {};
\node[hackennode] (e3) at (-.3,-1.1) {};
\node[hackennode] (c) at (1,1) {};
\node[right] at (1,1.25) {$c$};
\node[hackennode] (c1) at (1,0) {};
\node[hackennode] (e1) at (1,-.5) {};
\node[hackennode] (e2) at (1,-.8) {};
\node[hackennode] (e3) at (1,-1.1) {};
\node[hackennode] (c2) at (1,-1.5) {};
\node[hackennode] (c3) at (1,-2.5) {};
\node[hackennode] (e1) at (1,-2.75) {};
\node[hackennode] (e2) at (1,-3) {};
\node[hackennode] (e3) at (1,-3.25) {};
\node[hackennode] (e1) at (-3,-.5) {};
\node[hackennode] (e2) at (-3,-.8) {};
\node[hackennode] (e3) at (-3,-1.1) {};
\node[hackennode] (e1) at (1,2.25) {};
\node[hackennode] (e2) at (1,2.5) {};
\node[hackennode] (e3) at (1,2.75) {};

\draw[thick, blue] (w3) -- (a) -- (b);
\draw[thick, blue] (w3) -- (c) -- (c1);
\draw[thick, blue] (c2) -- (c3);
\draw[thick, blue] (b1) -- (b2);

\node[left] at (-2.5,2) {$n$};
\node[left] at (-2.5,1) {$n-1$};
\node[left] at (-2.5,0) {$n-2$};
\node[left] at (-2.5,-1.5) {$n-k+1$};
\node[left] at (-2.5,-2.5) {$n-k$};
\node[left] at (-2.5,-3.5) {$n-k-1$};


\draw[gray, dashed] (-2.5,2)--(2.5,2);
\draw[gray, dashed] (-2.5,1)--(2.5,1);
\draw[gray, dashed] (-2.5,0)--(2.5,0);
\draw[gray, dashed] (-2.5,-1.5)--(2.5,-1.5);
\draw[gray, dashed] (-2.5,-2.5)--(2.5,-2.5);
\draw[gray, dashed] (-2.5,-3.5)--(2.5,-3.5);

\end{tikzpicture}
\caption{A branch of length $k$ originating at vertex $a$.}
\label{branchfig}
\end{figure}

==> TauProofTikz.tex <==
 \begin{figure}[h]
 \centering
 \label{Tauprooffig}
\begin{tikzpicture}[thick,scale=0.6, every node/.style={scale=0.6}]

\draw[gray, dashed] (-5,2)--(5,2);
\draw[gray, dashed] (-5,1)--(5,1);
\draw[gray, dashed] (-5,0)--(5,0);
\draw[gray, dashed] (-5,-1.5)--(5,-1.5);
\draw[gray, dashed] (-5,-2.5)--(5,-2.5);
\draw[gray, dashed] (-5,-3.5)--(5,-3.5);
\draw[gray, dashed] (-5,-5)--(5,-5);
\draw[gray, dashed] (-5,-6)--(5,-6);
\draw[gray, dashed] (-5,-7)--(5,-7);

\node[left] at (-5,2) {$g_2 + k + 1$};
\node[left] at (-5,1) {$g_2 + k$};
\node[left] at (-5,0) {$g_2 + k - 1$};
\node[left] at (-5,-1.5) {$g_2 + 1$};
\node[left] at (-5,-2.5) {$g_2$};
\node[left] at (-5,-3.5) {$g_2 - 1$};
\node[left] at (-5,-5) {$g_1 + 1$};
\node[left] at (-5,-6) {$g_1$};
\node[left] at (-5,-7) {$g_1 - 1$};

\node[hackennode] (d11) at (-5.5,2.6) {};
\node[hackennode] (d12) at (-5.5,2.8) {};
\node[hackennode] (d13) at (-5.5,3) {};
\node[hackennode] (d21) at (-5.5,-1) {};
\node[hackennode] (d22) at (-5.5,-.8) {};
\node[hackennode] (d23) at (-5.5,-.6) {};
\node[hackennode] (d31) at (-5.5,-4.5) {};
\node[hackennode] (d32) at (-5.5,-4.3) {};
\node[hackennode] (d33) at (-5.5,-4.1) {};

%R(i+r+1)
\node[hackennode] (Ra1) at (-3,-6) {};
\node[hackennode] (Ra2) at (-3,-5) {};
\node[hackennode] (d31b) at (-3,-4.5) {};
\node[hackennode] (d32b) at (-3,-4.3) {};
\node[hackennode] (d33b) at (-3,-4.1) {};
\node[hackennode] (Ra3) at (-3,-3.5) {};
\node[hackennode] (Ra4) at (-3,-2.5) {};
\node[hackennode] (Ra5) at (-3,-1.5) {};
\node[hackennode] (d21b) at (-3,-1) {};
\node[hackennode] (d22b) at (-3,-.8) {};
\node[hackennode] (d23b) at (-3,-.6) {};
\node[hackennode] (Ra6) at (-3,0) {};
\node[hackennode] (Ra7) at (-3,1) {};
\node[hackennode] (Ra8) at (-3,2) {};
\node[hackennode] (d11b) at (-3,2.6) {};
\node[hackennode] (d12b) at (-3,2.8) {};
\node[hackennode] (d13b) at (-3,3) {};

\node[below] at (-3,-6.2) {$R_{i + r + 1}$};
\draw[thick, blue] (Ra1) -- (Ra2);
\draw[thick, blue] (Ra3) -- (Ra4) -- (Ra5);
\draw[thick, blue] (Ra6) -- (Ra7) -- (Ra8);

%R(j)
\node[hackennode] (Rb7) at (0,1) {};
\node[hackennode] (Rb8) at (0,2) {};
\node[hackennode] (d11c) at (0,2.6) {};
\node[hackennode] (d12c) at (0,2.8) {};
\node[hackennode] (d13c) at (0,3) {};

\node[below] at (0,.8) {$R_{j}$};
\draw[thick, blue] (Rb7) -- (Rb8);


%R(j+q+1)
\node[hackennode] (Rc4) at (3,-2.5) {};
\node[hackennode] (Rc5) at (3,-1.5) {};
\node[hackennode] (d21d) at (3,-1) {};
\node[hackennode] (d22d) at (3,-.8) {};
\node[hackennode] (d23d) at (3,-.6) {};
\node[hackennode] (Rc6) at (3,0) {};
\node[hackennode] (Rc7) at (3,1) {};
\node[hackennode] (Rc8) at (3,2) {};
\node[hackennode] (d11d) at (3,2.6) {};
\node[hackennode] (d12d) at (3,2.8) {};
\node[hackennode] (d13d) at (3,3) {};

\node[below] at (3,-2.7) {$R_{j+q+r}$};
\draw[thick, blue] (Rc4) -- (Rc5);
\draw[thick, blue] (Rc6) -- (Rc7) -- (Rc8);

\end{tikzpicture}

 \caption{Constructing $\Gamma_\tau$ when $\tau$ has $k$ consecutive negative ones preceded by $k$ consecutive positive ones.}
\end{figure}
